How Attentive are Graph Attention Networks?

Graph Attention Networks (GATs) are one of the most popular GNN architectures and are considered as the state-of-the-art architecture for representation learning with graphs. In GAT, every node attends to its neighbors given its own representation as the query. However, in this paper we show that GAT computes a very limited kind of attention: the ranking of the attention scores is unconditioned on the query node. We formally define this restricted kind of attention as static attention and distinguish it from a strictly more expressive dynamic attention. Because GATs use a static attention mechanism, there are simple graph problems that GAT cannot express: in a controlled problem, we show that static attention hinders GAT from even fitting the training data. To remove this limitation, we introduce a simple fix by modifying the order of operations and propose GATv2: a dynamic graph attention variant that is strictly more expressive than GAT. We perform an extensive evaluation and show that GATv2 outperforms GAT across 11 OGB and other benchmarks while we match their parametric costs. Our code is available at https://github.com/tech-srl/how_attentive_are_gats . GATv2 is available as part of the PyTorch Geometric library, the Deep Graph Library, and the TensorFlow GNN library.

==> biological_results.tex <==
	\begin{minipage}{0.48\textwidth}
    \centering
    \footnotesize
        \begin{tabular}{lrrr}
        \toprule
         & \multicolumn{1}{c}{\scriptsize{ENZYMES}} & \multicolumn{1}{c}{\scriptsize{NCI1}} & \multicolumn{1}{c}{\scriptsize{PROTEINS}} \\
         \midrule
		GAT$_{1h}$ & \textbf{68.3}\err{4.7} & 76.6\err{2.3}  & \textbf{73.9}\err{3.5} \\
         \dpgat{}$_{1h}$ & 67.3\err{4.6} & 75.7\err{2.1} & 72.6\err{4.1} \\
         \newgat{}$_{1h}$	   & 67.3\err{5.7} & \textbf{77.5}\err{1.1} & \textbf{73.9}\err{3.8}		\\
         \midrule
		GAT$_{8h}$ & \textbf{68.6}\err{5.9}& \textbf{77.0}\err{2.6} & 72.2\err{3.4}\\
        \dpgat{}$_{8h}$ & 66.3\err{6.2} & 73.7\err{3.2} & 73.0\err{2.8} \\
        \newgat{}$_{8h}$ & 66.2\err{5.6} & 76.6\err{2.6} & \textbf{73.5}\err{3.4}\\
\bottomrule
    \end{tabular}
    \captionof{table}{Average accuracy (30 runs$\pm$stdev) on biological benchmarks. ${\dagger}$ -- previously reported by \citet{errica2020fair}.}%
    \label{tab:bio-results}
	\end{minipage}

==> link-collab-table.tex <==
\begin{table*}[t]
    \centering
    \footnotesize
    \begin{tabu}{lcccccccc}
        \toprule
        \rowfont{\footnotesize}
            & \multicolumn{8}{c}{\textbf{ogbl-collab}}\\
        	& \multicolumn{2}{c}{Hits@10} & & \multicolumn{2}{c}{Hits@50} & &\multicolumn{2}{c}{Hits@100}\\         
\cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9}
\rowfont{\footnotesize}
        Model & \multicolumn{1}{c}{w/o val edges} & \multicolumn{1}{c}{w/ val edges} & & \multicolumn{1}{c}{w/o val edges}& \multicolumn{1}{c}{w/ val edges} & & \multicolumn{1}{c}{w/o val edges} & \multicolumn{1}{c}{w/ val edges} \\
        \midrule
        \normalsize{GAT$_{1h}$} & \textbf{18.86}$\pm$\scriptsize{1.91} & \textbf{19.03}$\pm$\scriptsize{3.32} & & 39.32$\pm$\scriptsize{3.26} & 48.10$\pm$\scriptsize{4.80} & & 47.31$\pm$\scriptsize{2.74} & 57.59$\pm$\scriptsize{2.97} \\
        \normalsize{\newgat{}$_{1h}$} & 17.67$\pm$\scriptsize{3.39} & 16.36$\pm$\scriptsize{4.18} & & 42.00$\pm$\scriptsize{2.40} & 48.02$\pm$\scriptsize{2.77} & & 49.70$\pm$\scriptsize{1.80} & 57.96$\pm$\scriptsize{1.82} \\
        \normalsize{\newgat{}$_{1h}$ 2 mat} & 16.87$\pm$\scriptsize{2.21} & 16.63$\pm$\scriptsize{3.12} & & 42.60$\pm$\scriptsize{2.22} & 50.07$\pm$\scriptsize{2.01} & & 50.79$\pm$\scriptsize{2.07} & 60.37$\pm$\scriptsize{1.72} \\
        \normalsize{\dpgat{}$_{1h}$} & 18.85$\pm$\scriptsize{3.60} & 16.53$\pm$\scriptsize{4.08} & & \textbf{44.15}$\pm$\scriptsize{1.59} & \textbf{49.61}$\pm$\scriptsize{3.16} & &  \textbf{51.28}$\pm$\scriptsize{1.27} & \textbf{59.74}$\pm$\scriptsize{1.71} \\
        \midrule
        \normalsize{GAT$_{8h}$} & 19.73$\pm$\scriptsize{1.84} & 20.74$\pm$\scriptsize{5.23} & & 42.37$\pm$\scriptsize{2.99} & 46.63$\pm$\scriptsize{2.80} & & 49.62$\pm$\scriptsize{2.44} & 56.57$\pm$\scriptsize{1.99} \\
        \normalsize{\newgat{}$_{8h}$} & 20.21$\pm$\scriptsize{2.96} & 20.94$\pm$\scriptsize{5.23} & & 42.85$\pm$\scriptsize{2.64} & 49.70$\pm$\scriptsize{3.08} & & 50.18$\pm$\scriptsize{1.80} & 59.00$\pm$\scriptsize{2.32} \\
        \normalsize{\newgat{}$_{8h}$ 2 mat} & 20.58$\pm$\scriptsize{4.26} & 19.40$\pm$\scriptsize{4.09} & & 44.47$\pm$\scriptsize{2.77} & 50.93$\pm$\scriptsize{3.07} & & 51.64$\pm$\scriptsize{2.30} & 60.06$\pm$\scriptsize{2.16} \\
        \normalsize{\dpgat{}$_{8h}$} & \textbf{31.82}$\pm$\scriptsize{2.89} & \textbf{32.48}$\pm$\scriptsize{5.48} & & \textbf{48.99}$\pm$\scriptsize{0.70} & \textbf{56.90}$\pm$\scriptsize{1.45} & &  \textbf{54.91}$\pm$\scriptsize{0.48} & \textbf{63.27}$\pm$\scriptsize{0.77} \\

        \bottomrule
    \end{tabu}
    \caption{Average Hits@$K$, for $K\in\{10,50,100\}$ with or without validation edges in test time (10 runs$\pm$std) on \textbf{ogbl-collab} dataset \citep{hu2020open}.}
    \label{tab:collab-results}
\end{table*} 

==> link-ddi-citation2-table.tex <==
\begin{figure}
	\begin{minipage}[t]{0.48\textwidth}
    \centering
    \footnotesize
    \begin{tabu}{llll}
        \toprule
            & \multicolumn{3}{c}{\textbf{ogbl-ddi}}\\
        	Model & \multicolumn{1}{c}{Hits@10} & \multicolumn{1}{c}{Hits@20} &\multicolumn{1}{c}{Hits@30}\\         
        \midrule
        \normalsize{GAT$_{1h}$} & 27.00$\pm$\scriptsize{7.93}  & \textbf{51.92}$\pm$\scriptsize{6.70} & 59.93$\pm$\scriptsize{8.37} \\
        \normalsize{\newgat{}$_{1h}$} & 23.88$\pm$\scriptsize{10.88} & 38.83$\pm$\scriptsize{8.57} & 55.02$\pm$\scriptsize{10.10} \\
        \normalsize{\newgat{}$_{1h}$ 2 mat} & 23.40$\pm$\scriptsize{5.46} & 39.30$\pm$\scriptsize{7.23} & 53.67$\pm$\scriptsize{7.68} \\
        \normalsize{\dpgat{}$_{1h}$} & \textbf{29.84}$\pm$\scriptsize{8.31} & 50.59$\pm$\scriptsize{7.51} &  \textbf{65.14}$\pm$\scriptsize{3.81} \\
        \midrule        
        \normalsize{GAT$_{8h}$} & \textbf{25.39}$\pm$\scriptsize{12.26} & \textbf{50.81}$\pm$\scriptsize{6.67} & 60.69$\pm$\scriptsize{5.52} \\
        \normalsize{\newgat{}$_{8h}$} & 21.38$\pm$\scriptsize{9.16} & 34.60$\pm$\scriptsize{11.21} & 49.89$\pm$\scriptsize{9.31} \\
        \normalsize{\newgat{}$_{8h}$ 2 mat} & 27.16$\pm$\scriptsize{13.82} & 44.06$\pm$\scriptsize{12.87} & 53.87$\pm$\scriptsize{12.30} \\
        \normalsize{\dpgat{}$_{8h}$} & 25.35$\pm$\scriptsize{7.51} & 47.91$\pm$\scriptsize{12.06} &  \textbf{63.07}$\pm$\scriptsize{6.31} \\
        \bottomrule
    \end{tabu}
        \captionof{table}{Average Hits@$K$, for $K\in\{10,20,30\}$ (10 runs$\pm$std) on \textbf{ogbl-ddi} dataset.}
     
        \label{tab:ddi-results}
	\end{minipage}
    \hfill
	\begin{minipage}[t]{0.40\textwidth}
    \centering
    \footnotesize
    \begin{tabular}{lc}
        \toprule
        Model             & \textbf{ogbl-citation2}\\ 
        \midrule
        \normalsize{GAT$_{1h}$}      & 79.84$\pm$\scriptsize{0.19} \\ 
        \normalsize{\newgat{}$_{1h}$}  & \textbf{80.33}$\pm$\scriptsize{0.13} \\ 
        \normalsize{\dpgat{}$_{1h}$}    & 80.31$\pm$\scriptsize{0.21} \\  
        \midrule
        \normalsize{GAT$_{8h}$}     & 75.95$\pm$\scriptsize{1.31} \\ 
        \normalsize{\newgat{}$_{8h}$}  & \textbf{80.14}$\pm$\scriptsize{0.71} \\ 
        \normalsize{\dpgat{}$_{8h}$}    & 79.64$\pm$\scriptsize{0.42} \\  
        \bottomrule
        \end{tabular}
        \captionof{table}{Average Mean Reciprocal Rank (MRR) (10 runs$\pm$std) on \textbf{ogbl-citation2} dataset.}
 
        \label{tab:citation2-results}
	\end{minipage}
\end{figure}

==> link-tables-dp.tex <==
\begin{table*}[h!]
\caption{Average Hits@50 %
(\Cref{tab:collab-results}) and mean reciprocal rank (MRR) (\Cref{tab:citation2-results}) in link-prediction benchmarks from OGB (10 runs$\pm$std). 
${\dagger}$ -- previously reported by \citet{hu2020open}.
}
    \centering
	\begin{subtable}{0.6\textwidth}
    \centering
    \footnotesize
    \begin{tabu}{llcc}
        \toprule
        \rowfont{\footnotesize}
            & & \multicolumn{2}{c}{\textbf{ogbl-collab}}\\
        & Model & \multicolumn{1}{c}{w/o val edges}& \multicolumn{1}{c}{w/ val edges} \\
        \midrule
        \multirow{2}{*}{\shortstack[c]{No-\vphantom{$^{\dagger}$}\\Attention}}
        & GCN$^{\dagger}$ & 44.75\err{1.07} & 47.14\err{1.45} \\
        & GraphSAGE$^{\dagger}$ & 48.10\err{0.81} & 54.63\err{1.12} \\
        \midrule
        \multirow{2}{*}{\shortstack[c]{GAT}} 
        & \normalsize{GAT$_{1h}$} & 39.32\err{3.26} & 48.10\err{4.80} \\
        & \normalsize{GAT$_{8h}$} & 42.37\err{2.99} & 46.63\err{2.80} \\
        \midrule
        \multirow{2}{*}{\shortstack[c]{\dpgat{}}} 
        & \normalsize{\dpgat{}$_{1h}$} & 44.15\err{1.59} & 49.61\err{3.16} \\
        & \normalsize{\dpgat{}$_{8h}$} & \textbf{48.99}\err{0.70} & \textbf{56.90}\err{1.45} \\
        \midrule
        \multirow{2}{*}{\shortstack[c]{\newgat{}}} 
        & \normalsize{\newgat{}$_{1h}$} & 42.00\err{2.40} & 48.02\err{2.77} \\
        & \normalsize{\newgat{}$_{8h}$} & 42.85\err{2.64} & 49.70\err{3.08} \\
        \bottomrule
    \end{tabu}
    \caption{}
    \label{tab:collab-results-dp}
	\end{subtable}
	\begin{subtable}{0.15\textwidth}
    \centering
    \footnotesize
    \begin{tabular}{c}
        \toprule
        \textbf{ogbl-citation2}\\ 
        \\
        \midrule
        80.04\vphantom{$^{\dagger}$}\err{0.25} \\
        \textbf{80.44}\vphantom{$^{\dagger}$}\err{0.10} \\
        \midrule
        79.84\err{0.19} \\ 
        75.95\err{1.31} \\ 
        \midrule
        80.31\err{0.21} \\  
        79.64\err{0.42} \\ 
        \midrule
        80.33\err{0.13} \\ 
        80.14\err{0.71} \\ 
        \bottomrule
        \end{tabular}
        \caption{}
         \label{tab:citation2-results-dp}
	\end{subtable}

\label{tab:link-results-dpgat-dp}
\end{table*}


==> node-geom-table.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{lcccccc}
        \toprule
        Model            & \textbf{Cornel}                      & \textbf{Texas}                       & \textbf{Wisconsin}                   & \textbf{Actor}                       & \textbf{Squirel}                     & \textbf{Chameleon}      
        \\ 
        \midrule
        GAT$_{\text{1 head}}$     & 57.84$\pm$\scriptsize{4.22}          & 58.38$\pm$\scriptsize{4.39}          & 51.76$\pm$\scriptsize{5.56}          & 26.93$\pm$\scriptsize{1.19}          & 30.08$\pm$\scriptsize{1.70}          & 41.47$\pm$\scriptsize{2.23}          \\ 
        GAT$_{\text{4 heads}}$    & 55.95$\pm$\scriptsize{4.37}          & 56.49$\pm$\scriptsize{5.05}          & \textbf{53.14}$\pm$\scriptsize{4.42} & 27.91$\pm$\scriptsize{1.17}          & \textbf{30.33}$\pm$\scriptsize{1.08} & \textbf{43.66}$\pm$\scriptsize{2.91} \\ 
        GAT$_{\text{8 heads}}$    & 53.51$\pm$\scriptsize{6.82}          & 55.41$\pm$\scriptsize{4.40}          & 48.82$\pm$\scriptsize{3.87}          & \textbf{28.14}$\pm$\scriptsize{0.82} & 30.09$\pm$\scriptsize{1.10}          & 43.36$\pm$\scriptsize{2.11}          \\ 
        \midrule
        \newgat$_{\text{1 head}}$ & 58.38$\pm$\scriptsize{5.01}          & \textbf{58.38}$\pm$\scriptsize{4.22} & 50.59$\pm$\scriptsize{6.49}          & 26.98$\pm$\scriptsize{1.29}          & 29.76$\pm$\scriptsize{1.80}          & 41.29$\pm$\scriptsize{2.16}          \\ 
        \dpgat{}$_{\text{1 head}}$   & \textbf{59.19}$\pm$\scriptsize{4.59} & 58.11$\pm$\scriptsize{4.23}          & 51.57$\pm$\scriptsize{4.64}          & 26.18$\pm$\scriptsize{1.38}          & 26.76$\pm$\scriptsize{1.42}          & 40.81$\pm$\scriptsize{2.25}          \\  
        \midrule
        \newgat$_{\text{8 heads}}$& 54.86$\pm$\scriptsize{5.93}          & 56.76$\pm$\scriptsize{4.52}          & 51.96$\pm$\scriptsize{4.49}          & 27.89$\pm$\scriptsize{0.87}          & 29.88$\pm$\scriptsize{1.11}          & 43.40$\pm$\scriptsize{2.39}          \\ 
        \dpgat{}$_{\text{8 heads}}$  & 54.86$\pm$\scriptsize{5.55}          & 54.32$\pm$\scriptsize{7.20}          & 50.78$\pm$\scriptsize{4.34}          & 28.32$\pm$\scriptsize{1.07}          & 26.35$\pm$\scriptsize{1.86}          & 39.78$\pm$\scriptsize{2.58}          \\  
        \bottomrule
    \end{tabular}

    \caption{Average acuuracy (10 different splits$\pm$std) on WebKB, Actor \citep{tang2009social} and Wikipedia \citep{rozemberczki2019multi} node prediction datasets.}
 
    \label{tab:node-geomgcn-results}
\end{table}

==> repro-statement.tex <==
\section*{Reproducibility Statement}
This paper is completely reproducible:
\begin{itemize}
	\item PyTorch Geometric and Deep Graph Library (DGL) implementations of our \newgat{} layer itself are included in the supplementary material.
	\item A proof for \Cref{theorem:monotonic} is provided in \Cref{subsec:limitation}.
	\item A proof for \Cref{theorem:dynamic} is provided in \Cref{sec:proof-dynamic}.
	\item \Cref{theorem:dpgat} and its proof are provided in \Cref{sec:dpgat-proof}.
	\item All the datasets that we used are publicly available,  except for the new synthetic \kchoose{} benchmark, which we will make publicly available, to serve as a testbed for future graph attention mechanisms. Dataset statistics are available in \Cref{sec:stats}.
	\item All experiments with public datasets were implemented using existing frameworks, slightly adapted to include the new \newgat{}. We repeated every experiment multiple times using different random seeds, as detailed in each figure's caption. Standard deviation for the experiments with QM9 (\Cref{tab:qm-results}) are shown in \Cref{sec:additional-qm} and \Cref{tab:qm-results-appendix}. All training details are available in \Cref{sec:training}. 
	\item Additional results for \kchoose{}, comparing \newgat{} with GIN empirically, are shown in \Cref{sec:additional-kchoose} and \Cref{fig:kchoose-results-additional}.
	\item A detailed time- and parameteric-complexity analysis is provided in \Cref{sec:complexity}.
\end{itemize}


